A Theory of PAC Learnability under Transformation Invariances

Transformation invariances are present in many real-world problems. For example, image classification is usually invariant to rotation and color transformation: a rotated car in a different color is still identified as a car. Data augmentation, which adds the transformed data into the training set and trains a model on the augmented data, is one commonly used technique to build these invariances into the learning process. However, it is unclear how data augmentation performs theoretically and what the optimal algorithm is in presence of transformation invariances. In this paper, we study PAC learnability under transformation invariances in three settings according to different levels of realizability: (i) A hypothesis fits the augmented data; (ii) A hypothesis fits only the original data and the transformed data lying in the support of the data distribution; (iii) Agnostic case. One interesting observation is that distinguishing between the original data and the transformed data is necessary to achieve optimal accuracy in setting (ii) and (iii), which implies that any algorithm not differentiating between the original and transformed data (including data augmentation) is not optimal. Furthermore, this type of algorithms can even "harm" the accuracy. In setting (i), although it is unnecessary to distinguish between the two data sets, data augmentation still does not perform optimally. Due to such a difference, we propose two combinatorial measures characterizing the optimal sample complexity in setting (i) and (ii)(iii) and provide the optimal algorithms.

==> section/app_eg_hurt.tex <==
%!TEX root = ../main.tex
\section{An example of $\dim(\cH,\cG) \gg \vcd(\cH)$}\label{app:eg-hurt}
\begin{example}
    For any $d>0$, let $\cX = \{\pm 1\}\times \{\be_i|i\in [2d]\}\subset \R^{2d+1}$, $\cH = \{x_1> 0, x_1\leq 0\}$ and $\cG = \{I_{2d+1}, I_{2d+1}-2\diag(\be_1)\}$ (i.e., the cyclic group generated by flipping the sign of $x_1$).
    It is easy to check that $\vcd(\cH) = 1$.
    Let $X = \{(1,\be_1), (1,\be_2),\ldots,(1,\be_{2d})\}$ and then the orbits generated from $X$ are $\bphi = \{\{(-1,\be_i),(1,\be_i)\}|i\in [2d]\}\}$.
    Every labeling $\bff\in \cY^{2d}$, if $\sum_{i\in [2d]}f_i$ is odd, let $\bx_\bff = ((2f_i-1,\be_i))_{i=1}^{2d}$; if $\sum_{i\in [2d]}f_i$ is even, let $\bx_f = ((1-2f_i,\be_i))_{i=1}^{2d}$.
    It is direct to check that $(\bff,\bx_\bff)\in B(\cH,\cG,\bphi)$ for all $\bff\in \cY^{2d}$.
    Then for all $i\in [2d]$, $\bff\oplus \bg=\be_i$ implies $x_{\bff,i}=x_{\bg,i}$.
    Hence, $\dim(\cH,\cG) = 2d$, where $d$ can be an arbitrary positive integer.
    According to Theorem~\ref{thm:re-mu-dim}, we have $\mu(\cH,\cG)\geq d$.
\end{example}
